Early Warning Software for Emergency Department Crowding

Emergency department (ED) crowding is a well-recognized threat to patient safety and it has been repeatedly associated with increased mortality. Accurate forecasts of future service demand could lead to better resource management and has the potential to improve treatment outcomes. This logic has motivated an increasing number of research articles but there has been little to no effort to move these findings from theory to practice. In this article, we present first results of a prospective crowding early warning software, that was integrated to hospital databases to create real-time predictions every hour over the course of 5 months in a Nordic combined ED using Holt-Winters' seasonal methods. We showed that the software could predict next hour crowding with a nominal AUC of 0.98 and 24 hour crowding with an AUC of 0.79 using simple statistical models. Moreover, we suggest that afternoon crowding can be predicted at 1 p.m. with an AUC of 0.84.

==> crowding_dist_daily.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Crowding &  Severe crowding \\
datetime &           &                  \\
\midrule
0        &      29.5 &              5.7 \\
1        &       7.6 &              2.9 \\
2        &      16.2 &              1.9 \\
3        &       9.5 &              0.0 \\
4        &      20.0 &              0.0 \\
5        &       2.9 &              1.0 \\
6        &       2.9 &              0.0 \\
\bottomrule
\end{tabular}


==> crowding_dist_hourly.tex <==
\begin{tabular}{lrr}
\toprule
{} &  Proportion &  Cumulative \\
datetime &             &             \\
\midrule
0        &         0.0 &         0.0 \\
1        &         0.0 &         0.0 \\
2        &         0.0 &         0.0 \\
3        &         0.0 &         0.0 \\
4        &         0.0 &         0.0 \\
5        &         0.0 &         0.0 \\
6        &         0.0 &         0.0 \\
7        &         0.0 &         0.0 \\
8        &         0.0 &         0.0 \\
9        &         0.0 &         0.0 \\
10       &         0.0 &         0.0 \\
11       &         0.0 &         0.0 \\
12       &         0.0 &         0.0 \\
13       &         0.0 &         0.0 \\
14       &         1.9 &         1.9 \\
15       &         5.7 &         7.6 \\
16       &        13.3 &        20.9 \\
17       &        21.0 &        41.9 \\
18       &        21.9 &        63.8 \\
19       &        11.4 &        75.2 \\
20       &        10.5 &        85.7 \\
21       &         7.6 &        93.3 \\
22       &         5.7 &        99.0 \\
23       &         1.0 &       100.0 \\
\bottomrule
\end{tabular}


==> horizonwise_metrics_hourly_t88.tex <==
\begin{tabular}{ccccccccc}
\toprule
            & model &  AHWM &  HWDM &  MHWM \\
metric & horizon &       &       &       \\
\midrule
accuracy & 1  &  0.97 &  0.97 &  0.97 \\
            & 2  &  0.97 &  0.97 &  0.97 \\
            & 3  &  0.97 &  0.96 &  0.96 \\
            & 4  &  0.96 &  0.96 &  0.96 \\
            & 5  &  0.96 &  0.95 &  0.95 \\
            & 6  &  0.96 &  0.94 &  0.94 \\
            & 7  &  0.96 &  0.93 &  0.93 \\
            & 8  &  0.96 &  0.93 &  0.93 \\
            & 9  &  0.96 &  0.92 &  0.92 \\
            & 10 &  0.96 &  0.91 &  0.91 \\
            & 11 &  0.96 &  0.90 &  0.91 \\
            & 12 &  0.96 &  0.90 &  0.90 \\
            & 13 &  0.96 &  0.89 &  0.89 \\
            & 14 &  0.95 &  0.88 &  0.88 \\
            & 15 &  0.95 &  0.88 &  0.88 \\
            & 16 &  0.94 &  0.88 &  0.88 \\
            & 17 &  0.94 &  0.88 &  0.89 \\
            & 18 &  0.94 &  0.89 &  0.89 \\
            & 19 &  0.94 &  0.90 &  0.90 \\
            & 20 &  0.94 &  0.90 &  0.91 \\
            & 21 &  0.93 &  0.91 &  0.91 \\
            & 22 &  0.93 &  0.91 &  0.91 \\
            & 23 &  0.93 &  0.91 &  0.91 \\
            & 24 &  0.93 &  0.92 &  0.92 \\
auc & 1  &  0.99 &  0.98 &  0.99 \\
            & 2  &  0.97 &  0.97 &  0.97 \\
            & 3  &  0.96 &  0.96 &  0.96 \\
            & 4  &  0.95 &  0.94 &  0.95 \\
            & 5  &  0.94 &  0.93 &  0.93 \\
            & 6  &  0.93 &  0.91 &  0.92 \\
            & 7  &  0.92 &  0.90 &  0.91 \\
            & 8  &  0.91 &  0.89 &  0.90 \\
            & 9  &  0.91 &  0.89 &  0.89 \\
            & 10 &  0.91 &  0.89 &  0.89 \\
            & 11 &  0.90 &  0.87 &  0.88 \\
            & 12 &  0.87 &  0.86 &  0.86 \\
            & 13 &  0.85 &  0.85 &  0.85 \\
            & 14 &  0.84 &  0.83 &  0.83 \\
            & 15 &  0.82 &  0.81 &  0.81 \\
            & 16 &  0.81 &  0.80 &  0.79 \\
            & 17 &  0.81 &  0.79 &  0.80 \\
            & 18 &  0.81 &  0.79 &  0.79 \\
            & 19 &  0.81 &  0.79 &  0.79 \\
            & 20 &  0.82 &  0.80 &  0.81 \\
            & 21 &  0.82 &  0.80 &  0.81 \\
            & 22 &  0.81 &  0.80 &  0.81 \\
            & 23 &  0.80 &  0.79 &  0.80 \\
            & 24 &  0.79 &  0.79 &  0.79 \\
f1 & 1  &  0.62 &  0.60 &  0.60 \\
            & 2  &  0.48 &  0.48 &  0.46 \\
            & 3  &  0.41 &  0.43 &  0.40 \\
            & 4  &  0.37 &  0.37 &  0.34 \\
            & 5  &  0.29 &  0.32 &  0.35 \\
            & 6  &  0.26 &  0.28 &  0.30 \\
            & 7  &  0.18 &  0.25 &  0.26 \\
            & 8  &  0.13 &  0.26 &  0.25 \\
            & 9  &  0.09 &  0.24 &  0.24 \\
            & 10 &  0.07 &  0.21 &  0.20 \\
            & 11 &  0.04 &  0.21 &  0.20 \\
            & 12 &  0.02 &  0.20 &  0.18 \\
            & 13 &  0.03 &  0.16 &  0.17 \\
            & 14 &  0.03 &  0.15 &  0.15 \\
            & 15 &  0.04 &  0.14 &  0.14 \\
            & 16 &  0.07 &  0.14 &  0.12 \\
            & 17 &  0.07 &  0.14 &  0.15 \\
            & 18 &  0.08 &  0.14 &  0.14 \\
            & 19 &  0.09 &  0.16 &  0.12 \\
            & 20 &  0.09 &  0.14 &  0.13 \\
            & 21 &  0.08 &  0.12 &  0.12 \\
            & 22 &  0.06 &  0.09 &  0.06 \\
            & 23 &  0.09 &  0.10 &  0.07 \\
            & 24 &  0.07 &  0.11 &  0.09 \\
sensitivity & 1  &  0.60 &  0.57 &  0.55 \\
            & 2  &  0.45 &  0.46 &  0.44 \\
            & 3  &  0.36 &  0.42 &  0.38 \\
            & 4  &  0.31 &  0.37 &  0.34 \\
            & 5  &  0.22 &  0.34 &  0.39 \\
            & 6  &  0.19 &  0.32 &  0.36 \\
            & 7  &  0.12 &  0.33 &  0.34 \\
            & 8  &  0.09 &  0.37 &  0.37 \\
            & 9  &  0.06 &  0.37 &  0.36 \\
            & 10 &  0.04 &  0.36 &  0.33 \\
            & 11 &  0.02 &  0.37 &  0.36 \\
            & 12 &  0.01 &  0.37 &  0.33 \\
            & 13 &  0.02 &  0.31 &  0.33 \\
            & 14 &  0.02 &  0.31 &  0.29 \\
            & 15 &  0.03 &  0.30 &  0.29 \\
            & 16 &  0.07 &  0.29 &  0.24 \\
            & 17 &  0.07 &  0.28 &  0.27 \\
            & 18 &  0.08 &  0.26 &  0.25 \\
            & 19 &  0.09 &  0.28 &  0.19 \\
            & 20 &  0.08 &  0.22 &  0.19 \\
            & 21 &  0.07 &  0.17 &  0.17 \\
            & 22 &  0.06 &  0.12 &  0.07 \\
            & 23 &  0.09 &  0.12 &  0.09 \\
            & 24 &  0.07 &  0.12 &  0.11 \\
specificity & 1  &  0.99 &  0.99 &  0.99 \\
            & 2  &  0.99 &  0.98 &  0.98 \\
            & 3  &  0.99 &  0.98 &  0.98 \\
            & 4  &  0.99 &  0.98 &  0.98 \\
            & 5  &  0.99 &  0.97 &  0.97 \\
            & 6  &  0.99 &  0.96 &  0.96 \\
            & 7  &  0.99 &  0.95 &  0.95 \\
            & 8  &  0.99 &  0.95 &  0.95 \\
            & 9  &  0.99 &  0.94 &  0.94 \\
            & 10 &  0.99 &  0.93 &  0.93 \\
            & 11 &  0.99 &  0.92 &  0.93 \\
            & 12 &  0.99 &  0.92 &  0.92 \\
            & 13 &  0.99 &  0.91 &  0.91 \\
            & 14 &  0.99 &  0.90 &  0.90 \\
            & 15 &  0.98 &  0.90 &  0.90 \\
            & 16 &  0.97 &  0.90 &  0.91 \\
            & 17 &  0.97 &  0.90 &  0.91 \\
            & 18 &  0.97 &  0.91 &  0.92 \\
            & 19 &  0.97 &  0.92 &  0.92 \\
            & 20 &  0.97 &  0.93 &  0.93 \\
            & 21 &  0.97 &  0.94 &  0.94 \\
            & 22 &  0.96 &  0.94 &  0.94 \\
            & 23 &  0.96 &  0.94 &  0.95 \\
            & 24 &  0.96 &  0.95 &  0.95 \\
\bottomrule
\end{tabular}


==> originwise_metrics_hourly_t88.tex <==
\begin{tabular}{ccccccccc}
\toprule
            & model &  AHWM &  HWDM &  MHWM \\
metric & origin &       &       &       \\
\midrule
accuracy & 1  &  0.65 &  0.57 &  0.57 \\
            & 2  &  0.63 &  0.56 &  0.56 \\
            & 3  &  0.63 &  0.55 &  0.58 \\
            & 4  &  0.67 &  0.54 &  0.57 \\
            & 5  &  0.71 &  0.54 &  0.49 \\
            & 6  &  0.68 &  0.56 &  0.57 \\
            & 7  &  0.70 &  0.59 &  0.60 \\
            & 8  &  0.71 &  0.61 &  0.63 \\
            & 9  &  0.69 &  0.69 &  0.65 \\
            & 10 &  0.72 &  0.70 &  0.66 \\
            & 11 &  0.74 &  0.74 &  0.76 \\
            & 12 &  0.72 &  0.76 &  0.78 \\
            & 13 &  0.77 &  0.77 &  0.79 \\
            & 14 &  0.76 &  0.76 &  0.80 \\
            & 15 &  0.79 &  0.83 &  0.79 \\
            & 16 &  0.80 &  0.77 &  0.79 \\
            & 17 &  0.74 &  0.74 &  0.75 \\
            & 18 &  0.72 &  0.72 &  0.72 \\
            & 19 &  0.71 &  0.70 &  0.68 \\
            & 20 &  0.71 &  0.67 &  0.68 \\
            & 21 &  0.66 &  0.68 &  0.69 \\
            & 22 &  0.68 &  0.63 &  0.63 \\
            & 23 &  0.69 &  0.59 &  0.60 \\
auc & 1  &  0.48 &  0.50 &  0.50 \\
            & 2  &  0.49 &  0.54 &  0.52 \\
            & 3  &  0.49 &  0.54 &  0.55 \\
            & 4  &  0.50 &  0.54 &  0.55 \\
            & 5  &  0.53 &  0.57 &  0.54 \\
            & 6  &  0.53 &  0.58 &  0.58 \\
            & 7  &  0.56 &  0.59 &  0.61 \\
            & 8  &  0.65 &  0.64 &  0.66 \\
            & 9  &  0.65 &  0.68 &  0.64 \\
            & 10 &  0.61 &  0.64 &  0.64 \\
            & 11 &  0.68 &  0.73 &  0.72 \\
            & 12 &  0.76 &  0.79 &  0.79 \\
            & 13 &  0.80 &  0.84 &  0.83 \\
            & 14 &  0.85 &  0.85 &  0.86 \\
            & 15 &  0.89 &  0.88 &  0.89 \\
            & 16 &  0.85 &  0.84 &  0.84 \\
            & 17 &  0.79 &  0.79 &  0.77 \\
            & 18 &  0.76 &  0.74 &  0.75 \\
            & 19 &  0.62 &  0.60 &  0.60 \\
            & 20 &  0.59 &  0.57 &  0.59 \\
            & 21 &  0.63 &  0.61 &  0.61 \\
            & 22 &  0.56 &  0.56 &  0.55 \\
            & 23 &  0.55 &  0.54 &  0.54 \\
f1 & 1  &  0.17 &  0.29 &  0.33 \\
            & 2  &  0.13 &  0.35 &  0.33 \\
            & 3  &  0.05 &  0.31 &  0.34 \\
            & 4  &  0.00 &  0.22 &  0.30 \\
            & 5  &  0.11 &  0.29 &  0.25 \\
            & 6  &  0.06 &  0.34 &  0.36 \\
            & 7  &  0.06 &  0.33 &  0.34 \\
            & 8  &  0.06 &  0.34 &  0.37 \\
            & 9  &  0.11 &  0.42 &  0.35 \\
            & 10 &  0.06 &  0.42 &  0.36 \\
            & 11 &  0.23 &  0.47 &  0.51 \\
            & 12 &  0.17 &  0.47 &  0.55 \\
            & 13 &  0.32 &  0.44 &  0.45 \\
            & 14 &  0.35 &  0.38 &  0.50 \\
            & 15 &  0.49 &  0.61 &  0.48 \\
            & 16 &  0.56 &  0.47 &  0.55 \\
            & 17 &  0.47 &  0.51 &  0.56 \\
            & 18 &  0.49 &  0.51 &  0.52 \\
            & 19 &  0.47 &  0.48 &  0.44 \\
            & 20 &  0.43 &  0.36 &  0.43 \\
            & 21 &  0.32 &  0.43 &  0.41 \\
            & 22 &  0.31 &  0.33 &  0.35 \\
            & 23 &  0.32 &  0.32 &  0.33 \\
sensitivity & 1  &  0.13 &  0.33 &  0.40 \\
            & 2  &  0.10 &  0.43 &  0.40 \\
            & 3  &  0.03 &  0.37 &  0.40 \\
            & 4  &  0.00 &  0.23 &  0.33 \\
            & 5  &  0.07 &  0.33 &  0.32 \\
            & 6  &  0.03 &  0.40 &  0.43 \\
            & 7  &  0.03 &  0.38 &  0.38 \\
            & 8  &  0.04 &  0.37 &  0.39 \\
            & 9  &  0.07 &  0.40 &  0.34 \\
            & 10 &  0.03 &  0.38 &  0.34 \\
            & 11 &  0.14 &  0.43 &  0.46 \\
            & 12 &  0.10 &  0.37 &  0.47 \\
            & 13 &  0.20 &  0.33 &  0.33 \\
            & 14 &  0.23 &  0.27 &  0.37 \\
            & 15 &  0.35 &  0.48 &  0.35 \\
            & 16 &  0.41 &  0.32 &  0.41 \\
            & 17 &  0.33 &  0.38 &  0.45 \\
            & 18 &  0.37 &  0.39 &  0.41 \\
            & 19 &  0.37 &  0.39 &  0.37 \\
            & 20 &  0.32 &  0.26 &  0.34 \\
            & 21 &  0.25 &  0.36 &  0.33 \\
            & 22 &  0.24 &  0.30 &  0.33 \\
            & 23 &  0.25 &  0.34 &  0.34 \\
specificity & 1  &  0.84 &  0.65 &  0.63 \\
            & 2  &  0.83 &  0.61 &  0.62 \\
            & 3  &  0.86 &  0.62 &  0.65 \\
            & 4  &  0.92 &  0.66 &  0.67 \\
            & 5  &  0.95 &  0.62 &  0.55 \\
            & 6  &  0.93 &  0.63 &  0.62 \\
            & 7  &  0.95 &  0.67 &  0.68 \\
            & 8  &  0.96 &  0.70 &  0.72 \\
            & 9  &  0.93 &  0.81 &  0.76 \\
            & 10 &  0.97 &  0.83 &  0.78 \\
            & 11 &  0.96 &  0.85 &  0.87 \\
            & 12 &  0.96 &  0.92 &  0.91 \\
            & 13 &  0.98 &  0.94 &  0.95 \\
            & 14 &  0.96 &  0.95 &  0.96 \\
            & 15 &  0.96 &  0.96 &  0.95 \\
            & 16 &  0.97 &  0.97 &  0.96 \\
            & 17 &  0.96 &  0.93 &  0.92 \\
            & 18 &  0.93 &  0.91 &  0.90 \\
            & 19 &  0.89 &  0.86 &  0.85 \\
            & 20 &  0.92 &  0.89 &  0.86 \\
            & 21 &  0.86 &  0.84 &  0.86 \\
            & 22 &  0.86 &  0.77 &  0.76 \\
            & 23 &  0.87 &  0.68 &  0.70 \\
\bottomrule
\end{tabular}

